A Conceptual Shift to Rectify a Defect in the Lorentz-Dirac Equation

In his analysis of the Classical Theory of Radiating Electrons, Dirac (1938) draws attention to the characteristic instability of solutions to the third order equation of motion. He remarks that changing the sign of the self-force eliminates the runaway solutions and gives `reasonable behaviour'. Dirac rejects such a change and proceeds with an ad hoc modification to the solutions of the initial value problem that is not consistent with the principle of causality. We argue that his reasons for rejecting the change of sign are invalid on both physical and mathematical grounds. The conceptual shift is to treat the physical particle as a composite of the source particle and the energy-momentum that is reversibly generated in its self-field by its motion. The reversibly generated energy in the self-field is interpreted as kinetic energy, and the changes that follow result in Dirac's change of sign. Several exact solutions to the new equation of motion and its linearisation are given. For a particle in orbital motion the self-force enables the applied force to generate radiation and kinetic energy in the self-field that results in an outward spiral motion. The theory is consistent with all well-established principles of physics, including the principle of causality.

==> rectifyLDE-macros.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{postulate}{Postulate}
\renewcommand{\thepostulate}{\Roman{postulate}}

%  special symbols
\newcommand*{\elec}{e}				% electron charge
\newcommand*{\tcl}{\tau_c}
\newcommand*{\fcl}{\nu_c}
\newcommand*{\V}[1]{\mathbf{#1}}
\newcommand*{\mx}[1]{{\mathsf{#1}}}
\DeclareMathOperator{\E}{\mathrm{e}}
\DeclareMathOperator{\I}{i}
\newcommand*{\SP}{\cdot}
\newcommand*{\bSP}{\boldsymbol{\SP}}
\newcommand*{\btimes}{\boldsymbol{\times}}
\DeclareMathOperator{\trace}{tr}
\newcommand*{\Trans}{\mathrm{T}}		% for transpose superscript
\DeclareMathOperator{\Heaviside}{\theta}	% Heaviside step function

% textstyle fractions
\newcommand*{\half}{{\textstyle{\frac{1}{2}}}}
\newcommand*{\third}{{\textstyle{\frac{1}{3}}}}
\newcommand*{\quarter}{{\textstyle{\frac{1}{4}}}}
\newcommand*{\twothirds}{{\textstyle{\frac{2}{3}}}}

% sub or super scripts
\newcommand*{\Sscript}[1]{{\mathrm{#1}}}

% derivative operators
\DeclareMathOperator{\gradient}{grad}
\newcommand*{\Grad}[1][]{\gradient_{#1}}
\DeclareMathOperator{\divergence}{div}
\newcommand*{\Div}[1][]{\divergence_{#1}}
\DeclareMathOperator{\curl}{curl}
\newcommand*{\Curl}[1][]{\curl_{#1}}
\DeclareMathOperator{\DIV}{\partial\,\SP}
\DeclareMathOperator{\GRAD}{\partial}
\newcommand*{\intD}[1][]{\mathrm{d}#1}
\newcommand*{\Dtl}[2][]{\displaystyle{\frac{\intD{#1}}{\intD{#2}}}}
\newcommand*{\Dpl}[2][]{\displaystyle{\frac{\partial{#1}}{\partial{#2}}}}
\newcommand*{\DDtl}[2][]{\displaystyle{\frac{\intD^2{#1}}{\intD{#2}^2}}}

% "dot on bracket" time derivative
\newcommand*{\updot}[1]{\bigl(#1\bigr)\mbox{\raise.5ex\hbox{$\V{\Dot{}}$}}}

% integral operator
\newcommand*{\integ}[4][0.8]{{\int_{#3}^{#4}{\hspace{-#1ex}}\intD{#2}\;}}


